Improved Pattern-Avoidance Bounds for Greedy BSTs via Matrix Decomposition

Greedy BST (or simply Greedy) is an online self-adjusting binary search tree defined in the geometric view ([Lucas, 1988; Munro, 2000; Demaine, Harmon, Iacono, Kane, Patrascu, SODA 2009). Along with Splay trees (Sleator, Tarjan 1985), Greedy is considered the most promising candidate for being dynamically optimal, i.e., starting with any initial tree, their access costs on any sequence is conjectured to be within $O(1)$ factor of the offline optimal. However, in the past four decades, the question has remained elusive even for highly restricted input. In this paper, we prove new bounds on the cost of Greedy in the ''pattern avoidance'' regime. Our new results include: The (preorder) traversal conjecture for Greedy holds up to a factor of $O(2^{\alpha(n)})$, improving upon the bound of $2^{\alpha(n)^{O(1)}}$ in (Chalermsook et al., FOCS 2015). This is the best known bound obtained by any online BSTs. We settle the postorder traversal conjecture for Greedy. The deque conjecture for Greedy holds up to a factor of $O(\alpha(n))$, improving upon the bound $2^{O(\alpha(n))}$ in (Chalermsook, et al., WADS 2015). The split conjecture holds for Greedy up to a factor of $O(2^{\alpha(n)})$. Key to all these results is to partition (based on the input structures) the execution log of Greedy into several simpler-to-analyze subsets for which classical forbidden submatrix bounds can be leveraged. Finally, we show the applicability of this technique to handle a class of increasingly complex pattern-avoiding input sequences, called $k$-increasing sequences. As a bonus, we discover a new class of permutation matrices whose extremal bounds are polynomially bounded. This gives a partial progress on an open question by Jacob Fox (2013).

==> header.tex <==
%\usepackage{fullpage}

\usepackage{booktabs}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{tikz}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{xspace}
%\usepackage{theorem}
\usepackage{graphicx}
\usepackage{mdframed}

\usepackage{comment}
\usepackage{mathdots}
\usepackage{xcolor}
%\usepackage{fullpage}
\usepackage{graphics}
\usepackage{colordvi}
\usepackage{color}
\usepackage{hyperref}
\usepackage{paralist}
\usepackage{bm}
\usepackage{mathpazo}
%\usepackage{eepic}
%\input{stdinc.tex}
\usepackage{cleveref}
\usepackage{float}
\usepackage{kbordermatrix}
\usepackage[ruled,vlined]{algorithm2e}


%\newtheorem{remark}{Remark}
\newcommand{\opt}{\mbox{\sf OPT}}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\lleft}{\mathsf{left}}
\newcommand{\rright}{\mathsf{right}}
\newcommand{\cost}{\mathsf{Cost}}
\newcommand{\oc}{\mathsf{OperationCost}}
\newcommand{\uc}{\mathsf{UpdateCost}}
\newcommand{\access}{\mathsf{access}}
\newcommand{\insertt}{\mathsf{insert}}
\newcommand{\delete}{\mathsf{delete}}

\newcommand{\lset}{{\mathcal L}}
\newcommand{\rset}{{\mathcal R}}
\newcommand{\cset}{{\mathcal C}}
\newcommand{\pset}{{\mathcal P}}
\newcommand{\bset}{{\mathcal B}}




\newcommand{\BOX}{\textsc{Box}}

\newcommand{\BOXR}{\textsc{BoxAndReset}}

\newcommand{\attention}[1]{\textcolor{red}{#1}}
\newcommand{\nidia}[1]{\textcolor{blue}{#1}}
\renewcommand{\opt}{{\sf OPT}\xspace} 
\newcommand{\mf}{{\sf MF}\xspace} 



\newcommand{\block}[1]{
  \underbrace{\begin{matrix}1 & \cdots & 1\end{matrix}}_{#1}
}

% \newenvironment{proof}{\par \noindent{\bf Proof:}}{\hfill\stopproof}
% \def\stopproof{\square}
% \def\square{\vbox{\hrule height.2pt\hbox{\vrule width.2pt height5pt \kern5pt
% \vrule width.2pt} \hrule height.2pt}}

\newenvironment{proofof}[1]{\noindent{\bf Proof of #1.}}%
        {\hspace*{\fill}$\Box$\par\vspace{4mm}}

\def\rddots#1{\cdot^{\cdot^{\cdot^{#1}}}}

\def\poooo#1{\marginpar{$\leftarrow$\fbox{P}}\footnote{$\Rightarrow$~{\sf #1 --po}}}

\newcommand{\gex}{{\sf gex}}

\def\po#1{\textcolor{red}{#1}}

\endinput

==> tex/123.tex <==
\newpage
\section{Avoid321 / 2-increasing} \label{section: 123}
Note that 2-increasing sequence may not be 2-decomposable. All touched points are partitioned into 3 sets
\begin{enumerate}
    \item $G_{BR^-}$ is a set of touched points $\langle a,t \rangle$ such that an area $(a,\infty)\times(-\infty,t)$ is input-empty.
    \item $G_{TL^-}$ is a set of touched points $\langle a,t \rangle$ such that an area $(-\infty,a)\times(t,\infty)$ is input-empty.
    \item $G_{BR^+,TL^+}$ is a set of touched points $\langle a,t \rangle$ such that each area $(a,\infty)\times(-\infty,t)$ and $(-\infty,a)\times(t,\infty)$ contains at least one input.
\end{enumerate}

\begin{claim}
$G_{BR^-}$ avoids $\kbordermatrix{
     & a & b &c&d \\
     t_3 &\ast&&\\
     t_2 &&  & \ast&  \\ 
    t_1& & \ast & & \ast}$.
\end{claim}
\begin{proof}
Since $\langle a,t_3 \rangle$ is in $G_{BR^-}$, then $(a,\infty)\times(-\infty,t_3)$ must be input-empty. This contradicts to Claim \ref{claim: inputRevealing} when consider $\langle b,t_1 \rangle$, $\langle c,t_2 \rangle$, and $\langle d,t_1 \rangle$.
\end{proof}

\begin{claim}
    $G_{TL^-}$ avoids $\kbordermatrix{
     & a & b  \\
     t_2 & \ast &   \\ 
    t_1&   & \ast }$.
\end{claim}
\begin{proof}
Since $\langle b,t_1 \rangle$ is in $G_{TL^-}$, then $(-\infty,b)\times(t_1,\infty)$ must be input-empty. This contradicts to Corollary \ref{corol: hidden} when consider $\langle b,t_1 \rangle$ and $\langle a,t_2 \rangle$. 
\end{proof}

\begin{claim}
$G_{BR^+,TL^+}$ avoids $\kbordermatrix{
     & a & b &c&d \\
     t_2 &\ast&  & \ast&  \\ 
    t_1& & \ast & & \ast}$.
\end{claim}
\begin{proof}
Let $p_1$ be an input point in $(-\infty,a)\times(t_2,\infty)$. Let $p_2$ be an input point in Claim \ref{claim: inputRevealing} when consider $\langle b,t_1 \rangle$, $\langle c,t_2 \rangle$, and $\langle d,t_1 \rangle$. Let $p_3$ be an input point in $(d,\infty)\times(-\infty,t_1)$. Since $p_1,p_2,p_3$ form 321-pattern, this contradicts to the fact that $X$ avoids 321.
\end{proof}

==> tex/figures.tex <==
\section{All Figures} 



==> tex/fullprelim.tex <==
\section{Full Preliminaries} \label{sec:full prelim}



\iffalse 

\subsection{For later use} 

\begin{definition} Notation for each type of point.
\begin{enumerate}
    \item Permutation input sequence $X$
    \item Touched point that is not input point $\times$% $\ast$
    \item Input point $\bullet$
%    \item Delete point  $\blacksquare$
    \item Delete min $\blacktriangleleft$, max $\blacktriangleright$
%    \item Insert point $\square$
    \item Insert min $\vartriangleleft$, max $\vartriangleright$
    \item Touched point $\ast$ % $\circledast$
 %   \item Coordinate $\langle,\rangle$
    \item Open and closed interval $(,)$     $[,]$
\end{enumerate}
\end{definition}
\fi 

==> tex/intro.tex <==

\section{Introduction} 

The dynamic optimality conjecture postulates that there exists an online binary search tree whose cost to serve any input sequence (search, insert, delete) is at most the optimal offline cost of any binary search trees.\footnote{We remark  subtle distinctions between variants of the dynamic optimality conjecture. In the most general form of the conjecture, the algorithm must start from (adversarially given) initial tree and handles any of the insert/delete/search requests. However, 
it is common to consider various simplified versions, such as, (i) the ``static'' dynamic optimality conjecture where the input only involves searches (without insert or delete), and (ii) the ``empty initial tree'' setting where we start with an empty BST and the input consists of a sequence of insertions.} The two most promising candidates for being dynamically optimal are Splay trees~\cite{sleator1985self} and Greedy~\cite{demaine2009geometry,munro2000competitiveness,lucas1988canonical}.
Despite continuing efforts for many decades (see, e.g.,the surveys and monographs~\cite{iacono2013pursuit,kozma2016binary,chalermsook2016landscape}), the conjecture remains wide open even for highly restricted corollaries of the conjecture. 

This paper focuses on Greedy's bounds for such corollaries through the lens of ``pattern avoidance'' (to be made precise later). Each of them is of independent interest and therefore has received a lot of attention in the literature. 

We describe below some of the most popular  conjectures that fall under the regime of pattern avoidance: 

\vspace{0.1in} 

\begin{minipage}{0.9\textwidth} 
\begin{mdframed}
{\bf Deque Conjecture: } For $m>n$, there exists an online binary search tree that, starting with any initial BST $R$ on $n$ keys, can serve $m$  operations {\sc InsertMin}, {\sc InsertMax}, {\sc DeleteMin}, {\sc DeleteMax} in $O(m)$ time.
\end{mdframed}
\end{minipage}


\vspace{0.1in} 

The deque conjecture has received a lot of attention for  the past three decades~\cite{sundar1992deque,pettie2007splay,DBLP:journals/corr/ChalermsookG0MS15a}. Splay has been shown to cost at most $O(m \alpha(n))$ by Sundar~\cite{sundar1992deque} and later $O(m \alpha^*(n))$ by Pettie~\cite{pettie2007splay}. 
Greedy is also known to cost $m 2^{O(\alpha(m,m+n))}$~\cite{DBLP:journals/corr/ChalermsookG0MS15a}.  

\vspace{0.1in} 


\begin{minipage}{0.9\textwidth} 
\begin{mdframed}
{\bf (Preorder) Traversal Conjecture: } There exists an online binary search trees that, starting with any initial BST on $n$ keys, for any input $X = (x_1,\ldots, x_n) \in [n]^n$ obtained by \textit{preorder} traversal of (potentially distinct) binary search tree $R$ on $[n]$, searches  $X$ with $O(n)$ cost.\footnote{More formally, $x_t$ is searched at time $t$ for all $t \in [n]$.}
\end{mdframed}
\end{minipage}

\vspace{0.1in} 

We refer to such a sequence $X$ that can be seen as a preorder traversal of some tree $R$ as {\em preorder traversal sequence.} The main, but often overlooked, part in the above definition is that we start with an arbitrary initial BST. Let us elaborate this point. 

One can ask popular conjectures of BST in two settings: (1) when the initial BST can be pre-processed or (2) when it cannot be pre-processed. There is a gap in our understanding of these two settings. For example, it is not know if Greedy's cost for preorder traversal is same in both the settings. 
In setting (1), Chalermsook et al. \cite{chalermsook2015pattern} showed that Greedy takes $O(n)$ for the preorder traversal {\em if preprocessing is allowed}. One can also solve this problem using the ideas in \cite{iacono2016weighted}. But in setting (2), the best known bound for online BSTs is by Greedy, which achieves the time bound of $n 2^{\alpha(n)^{O(1)}}$ (with a relatively large exponent). For Splay, some special cases have been considered by Levy and Tarjan~\cite{levy2019splaying}. However, it has remained open whether Splay's cost is $o(n\log n)$ for preorder traversals.  \footnote{The $O(n \log \log n)$ bound follows from Tango's trees\cite{demaine2007dynamic}.} In this paper all results abide setting 2.

\vspace{0.1in} 


\begin{minipage}{0.9\textwidth} 
\begin{mdframed}
{\bf (Postorder) Traversal Conjecture: } There exists an online binary search trees that, starting with any initial BST on $n$ keys, for any input $X = (x_1,\ldots, x_n) \in [n]^n$ obtained by \textit{postorder} traversal of (potentially distinct) binary search tree $R$ on $[n]$, searches  $X$ with $O(n)$ cost.
\end{mdframed}
\end{minipage}

\vspace{0.1in} 


Again using \cite{iacono2016weighted}, we can show that Greedy's cost for the  above problem is $O(n)$ if pre-processing is allowed. If preprocessing is not allowed, then postorder traversals have only been considered recently by Levy and Tarjan~\cite{levy2019splaying}, who showed that some special settings of postorder traversals cost $O(n)$. For Greedy, the upper bound of $n 2^{O(\alpha(n)^{O(1)})}$ follows from~\cite{chalermsook2015pattern}.  %\footnote{Sorrachai: Maybe mention Split Conjecture as well?} 

%A split operation {\sc Split}($a$) on BST $R$ searches and brings $a$ up to the root and deletes it, thus breaking the $R$ into two disjoint binary search trees.
Another BST operation that has been studied (besides search/insert/delete) is splitting. 
Given an initial binary search tree $R$ with $n$ keys, the split tree supports the operations {\sc Split}($i$) which moves $i$ to the root and then deletes it, leaving two independent binary search (split) trees.\footnote{This is a somewhat ``adversarial'' view of split tree, i.e., the initial BST is given to us adversarially. When we are allowed to choose $R$, there exists a BST that serves split operations in $O(n)$ time~\cite{demaine2007dynamic}, and Splay is known to cost $O(n \alpha(n))$ when $R$ is a path~\cite{lucas1988canonical}.}
Lucas~\cite{lucas1992competitiveness} made the following conjecture:  

\vspace{0.1in} 

\begin{minipage}{0.9\textwidth} 
\begin{mdframed}
{\bf Split Conjecture:}  There exists an online binary search tree that, starting with any initial tree with $n$ keys, serves a sequence of split operations in time $O(n)$. 
\end{mdframed}
\end{minipage}


\vspace{0.1in} 

The author showed that the split costs $O(n\alpha(n))$ in Splay trees when the initial tree is a path.   %the split conjecture follows from the dynamic optimality conjecture of Splay and analyzed some special cases. 
Resolving these conjectures (especially the first two) is considered the ``simplest'' step of dynamic optimality conjecture and yet has so far resisted attempts for three decades. %\footnote{Split Conjectures? and K-Increasing?}

\vspace{0.2in} 

\noindent 
{\bf Our results and broader perspectives:}  Our first main theorem made progress to the first two aforementioned conjectures, and completely settled the third conjecture for Greedy.  %\footnote{Sorrachai: Maybe summarize all results in a table? Also compare with previous results.}

\begin{theorem} \label{thm:main}
The following bounds hold for Greedy: 
\begin{enumerate}
    \item \label{item:main1} Starting with any initial BST $R$ with $n$ keys, Greedy serves $m$ operations of {\sc InsertMin}, {\sc InsertMax}, {\sc DeleteMin}, {\sc DeleteMax} with cost at most $O(m \alpha(n))$ assuming $m>n$. 
    
    \item \label{item:main2}Greedy searches any preorder traversal sequence with cost $O(n 2^{\alpha(n)})$. 
    
    \item \label{item:main3}Greedy searches any postorder traversal sequence with cost $O(n)$. 
    
  %  \item 
\end{enumerate}
\end{theorem}

\begin{remark}
The sequence for preorder and postorder is a permutation sequence of length $n$. For deque we consider any sequence of length $m>n$.
\end{remark}


\begin{remark}
In all our results we consider an initial tree $T$ before the execution of Greedy. If the initial tree is not given, then problems becomes much "easier" to solve. For example the cost of sequential access is $O(n)$ with initial tree and without initial tree but the proof structures are different~\cite{chalermsook2015pattern,fox2011upper}.
\end{remark}



%As a bonus, we show that Greedy can be used as a split tree  with cost $O(n2^{\alpha(n)})$.\footnote{We consider the following split problem: Given an initial binary search tree $R$ with $n$ keys, the split tree supports the operations {\sc Split}($i$) which moves $i$ to the root and then deletes it, leaving two independent binary search (split) trees. This is a somewhat ``adversarial'' view of split tree, i.e., the initial BST is given to us adversarially. When we are allowed to choose $R$, there exists a BST that serves split operations in $O(n)$ time~\cite{demaine2007dynamic}, and Splay is known to cost $O(n \alpha(n))$ when $R$ is a path~\cite{lucas1988canonical}.} 


\begin{table}[]
\centering


\begin{tabular}{lccc}
\toprule
          & \textbf{Previous known}               & \textbf{This paper}                                 & \textbf{Remark} \\ \hline
Deque          & $m2^{\alpha(m,m+n)}$ \cite{DBLP:journals/corr/ChalermsookG0MS15a}  & $O(m\alpha(n))$                     &   \Cref{thm:main}(\ref{item:main1})\\  \hline
Preorder       & $n2^{\alpha(n)^{O(1)}}$ \cite{chalermsook2015pattern} & $O(n2^{\alpha(n)})$                 & \Cref{thm:main}(\ref{item:main2}) \\  \hline
Postorder      & $n2^{\alpha(n)^{O(1)}}$ \cite{chalermsook2015pattern} & $O(n)$                              &\Cref{thm:main}(\ref{item:main3})  \\  \hline
Split          & -                       & $O(n2^{\alpha(n)})$                 &  \Cref{thm:main split}\\  \hline
$k$-Increasing & $n2^{O(k^2)}$   \cite{chalermsook2015pattern}       & $O(\min\{nk^{2}, nk \alpha(n) \})$ &  \Cref{thm:main k-dec} \\ \bottomrule
\end{tabular}
\caption{Main results for Greedy BSTs. \label{table:results}}
\end{table}
 

For split conjecture, we in fact prove that the maximum cost of Greedy's splitting is at most the cost of searching a preorder traversal and therefore our traversal bound directly gives an upper bound on Greedy's serving split tree operations.   

\begin{theorem}[Informal]
\label{thm:main split} For $n \in {\mathbb N}$, let ${\sf deldeq}(n)$  be the maximum possible costs of Greedy when serving deletion-only deque operations on $n$ keys, and  ${\sf preorder}(n)$ be the maximum cost

 when serving preorder search. Then, 
\[{\sf deldeq}(n) \leq {\sf split}(n) \leq {\sf preorder}(n).\] 
Consequently, Greedy can be used as a split tree with cost $O(n 2^{\alpha(n)})$.
\end{theorem}

As a consequence, the traversal conjecture implies the split conjecture, which implies the delete-only deque conjecture. The implication from traversal to split conjectures is not known for Splay trees; it is known that dynamic optimality conjecture for Splay  implies split conjecture for Splay~\cite{lucas1992competitiveness}.  

One can view this collection of conjectures as the dynamic optimality conjecture on restricted inputs, where the restriction on the input sequence is defined by pattern avoidance properties.  Pattern avoiding problems are interesting special cases of the dynamic optimality conjecture that have shown  interplay between extremal combinatorics and data structures. 


We now define pattern avoidance formally. Consider any input $X$.\footnote{It was argued in~\cite{demaine2007dynamic} that one can assume w.l.o.g. that the input is a permutation.} We say that $X=(x_1, x_2, \ldots, x_n)$ contains pattern $\pi = (\pi_1,\ldots, \pi_k)$ if there are indices $i_1 < \ldots < i_k$ such that the subsequence $(x_{i_1}, x_{i_2}, \ldots, x_{i_k})$  is order-isomorphic to $\pi$. 
Otherwise,  $X$ avoids $\pi$. 

The three conjectures can be (roughly) rephrased in this language as follows. For the preorder traversal conjecture, we are given an input permutation $X$ that avoids pattern $(2,3,1)$, and our goal is to show a binary search tree that searches this sequence with cost at most $O(n)$. For the postorder traversal conjecture, our goal is to search an input sequence that avoids $(1,3,2)$. For the deque conjecture, if we represent the (delete-only) input $X$ (where $x_t$ is the key deleted at time $t$), then $X$ avoids patterns $(2,3,1)$ and $(2,1,3)$. 
In this way, all these conjectures deal with size-$3$ pattern-avoiding input classes. 


Besides the small patterns, recent works have also started exploring the complexity of input classes that avoid patterns of growing sizes~\cite{chalermsook2015pattern,goyal2019better,chalermsook2016landscape}. 
See the thesis of Kozma~\cite{kozma2016binary} for more detail about this connection. 
Our second main result shows the improvement on a pattern-avoiding input class that allow patterns to be growing in terms of $k$. We say that an input $X$ is $k$-\textit{increasing} (respectively, $k$-\textit{decreasing}) if $X$ avoids $(k+1,k,k-1,\ldots,1)$ (respectively, $(1,2,\ldots,k,k+1)$). Note that $1$-increasing (1-decreasing) sequence corresponds to sequential sequences: $X = (1,\ldots,n)$ (or $X = (n,\ldots,1)$, respectively). The sequential sequence has been studied in the early days of the dynamic optimality conjecture~\cite{tarjan1985sequential,elmasry2004sequential} for splay and a bit more recently for Greedy~\cite{fox2011upper}. Note that $k$-increasing sequence and $k$-decreasing sequence are symmetric. 
%\footnote{We are interchangeably using k-inc/k-dec.}\footnote{Mention k-inc/k-dec are symmetric.} 

\begin{theorem}
\label{thm:main k-dec} 
For $k$-increasing or $k$-decreasing input $X$, Greedy serves input $X$ with cost at most $O(\min\{n k^{2}, nk\alpha(n)\})$. 
\end{theorem}

Previously, the best analysis of Greedy achieves the upper bound of $n 2^{O(k^2)}$~\cite{chalermsook2015pattern}, so this is an exponential improvement in the dependence on parameter $k$.  When $k = \omega( 2^{\alpha(n)})$, the new upper bound term $O(nk\alpha (n))$ also improves over the best known bound even for offline optimal BST algorithm, which is $O(nk\log k)$ \cite{chalermsook2015pattern}. \Cref{table:results} summarizes our main results. 


%We refer to sequences avoiding $(k+1,\ldots, 1)$ as $k$-increasing sequences. When $k=1$, the input is $X=(1,2,\ldots, n)$ which has been studied in the early days of the dynamic optimality conjecture~\cite{tarjan1985sequential,elmasry2004sequential} for splay and a bit more recently for Greedy~\cite{fox2011upper}.  \footnote{We are interchangeably using k-inc/k-dec.}\footnote{Mention k-inc/k-dec are symmetric.}

%\attention{TODO: Table of results} 


\vspace{0.2in} 

\noindent 
{\bf Overview of Techniques:} 
Our techniques contribute broadly to the line of work that attempt to leverage the power of extremal bounds in amortized analysis of data structures.
In the context of binary search trees, such attempts were pioneered by Pettie~\cite{pettie2007splay,pettie2010applications} and more recently extended by~\cite{chalermsook2015pattern}. 
We provide an overview of their techniques and discuss how our approaches extend and strengthen theirs. 


%The key idea of this approach is to connect Greedy's cost to the classical theory of forbidden matrices. 
Roughly speaking, forbidden submatrix theory is a collection of theorems of the following form: Let $\pi$ be a matrix (pattern), and ${\sf ex}(n, \pi)$ denotes the extremal bound which equals the maximum number of $1$s in any $n$-by-$n$ $0/1$ matrix that does not contain pattern $\pi$ (a matrix $M$ contains pattern $\pi$ if it is possible to obtain $\pi$ from $M$ by removing rows, columns, and turning ones into zeroes); see \Cref{fig:pattern}. This theory provides a collection of upper and lower bounds on ${\sf ex}(n,\pi)$ for many patterns $\pi$.  

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.27]{tex/Figures/patterncontain.JPG}
  \caption{An example that $M$ contains pattern $\pi_1$, but avoids $\pi_2$.\label{fig:pattern}} 
\end{figure}

Let $X \in [n]^n$ be an input. Denote by $M_X$ the matrix that ``encodes'' the execution log of the BST, that is, $M_X(i,j) =1$ if and only if the BST algorithm touches key $i$ at time $j$, implying that the number of $1$s in $M_X$ (denoted by $|M_X|$) is equal to the cost of the algorithm. 

The connection between BST and the theory of forbidden matrices (see, e.g., in~\cite{chalermsook2015pattern}) relies on a ``reduction statement'', which says that if $X$ avoids a pattern $\pi$ of size $k$, then the Greedy matrix $M_X$ avoids a (tensored) pattern $\pi'$ of size $3k$. Therefore, existing extremal bounds can be immediately used to upper bound $|M_X|$.   
Indeed, for preorder and postorder traversals (that avoid patterns of size $3$), $M_X$ avoids a pattern of size $9$. The bound of $n 2^{\alpha(n)^{O(1)}}$ follows from this generic reduction.
%The main open question in this line of work is whether the theory of forbidden matrices can be used to settle deque and traversal conjectures (see, e.g.,\cite{pettie2007splay}). 
It is an intriguing open question to further extend this technique to settle deque and/or traversal conjectures. 
However, there are various obstacles in doing so. 
For instance, the most straightforward attempt where we would like to prove directly that $M_X$ avoids a ``linear-cost pattern'' (i.e. pattern $\pi$ whose extremal bound ${\sf ex}(n,\pi) = O(n)$) would not work (a counter example  is provided in~\cite{chalermsook2015pattern}.)  

In this paper, we propose to break the Greedy matrix $G(X)$ into several matrices that are ``easier in different ways''. More formally, we write $G(X) = \sum_{i = 1}^{\ell} Q_i$ where matrices $Q_i$ are chosen based on the structures of $G(X)$ so that each $Q_i$  avoids a much smaller pattern $\pi_i$ (which can be different for distinct $i$). This would give the upper bound $|G(X)| \leq \sum_{i=1}^{\ell} {\sf ex}(n, \pi_i)$. All our results follow this framework. 
%We will use \Cref{thm:exbound} to derive extremal bounds of forbidden matrices. 


\begin{itemize}
    \item For ``deque'' input $X$, we have 
    \[|G(X)| \leq {\sf ex}\bigg(n,\kbordermatrix{
     &  &   & &  \\
      &  & 1 &   &  1 \\ 
    &  1  & &  1  &  }\bigg) + {\sf ex}\bigg(n, \kbordermatrix{
     &  &   & &  \\
      & 1 &  & 1  &   \\ 
    &   &1 &    & 1 }\bigg) + O(n)\] 
    
    which implies that $|G(X)| \leq O(n \alpha(n))$. We remark that, without the decomposition trick, the matrix $G(X)$ itself contains pattern $\kbordermatrix{
     &  &  & & &  \\
      & 1 & &1 && 1 \\ 
    &   & 1& & 1 &}$.  \attention{TODO: Give a counterexample in appendix.}  
    
    \item For preorder traversal input $X$, we have 
    \begin{eqnarray*}
      |G(X)|& \leq & {\sf ex}\bigg(n,\kbordermatrix{
     &  &   \\
     & 1 &   \\ 
    &   & 1 } \bigg) + {\sf ex}\bigg(n,  \kbordermatrix{
     & & &  \\
     & 1 & &1  \\ 
    &   & 1& } \bigg) + 2\cdot {\sf ex}\bigg(n, \kbordermatrix{
     &  &  & & &  \\
      & 1 & &1 && 1 \\ 
    &   & 1& & 1 &} \bigg) 
    \end{eqnarray*} 
    which impies that $|G(X)| \leq O(n 2^{\alpha(n)})$. 
    
    \item For postorder traversal input $X$, we have 
    \begin{eqnarray*}
      |G(X)|& \leq & {\sf ex}\bigg(n,\kbordermatrix{
     &  &   \\
     & 1 & 1  \\ 
    &   & 1 } \bigg) + {\sf ex}\bigg(n,  \kbordermatrix{
     & & &  \\
     & 1 & &1  \\ 
    &   & 1& } \bigg) +  2 \cdot {\sf ex}\bigg(n,  \kbordermatrix{
     & & &  \\
     &  & 1&  \\ 
    &  1 & & 1 } \bigg)
    \end{eqnarray*}
    which implies that $|G(X)| = O(n)$. 
\end{itemize}



Finally, we sketch the ideas to prove the upper bound of $O(n \cdot poly (k))$ when $X$ avoid $(1,2,\ldots, k)$. In~\cite{chalermsook2015pattern}, it was proved that $G(X)$ avoids a permutation pattern $\pi$ of size $O(k^2)$. This implies, using~\cite{CibulkaK17,marcus2004excluded}, that $|G(X)| \leq {\sf ex}(n,\pi) \leq n \cdot 2^{O(|\pi|)} \leq n \cdot 2^{O(k^2)}$. Without using the structure of $\pi$, the exponential dependence on $k$ is necessary~\cite{fox2013stanley}. 

In this paper, using our decomposition trick, we show that the matrix $G(X)$ can be decomposed into $k$ matrices, each avoiding a much simpler pattern of size $k+2$; in particular $|G(X)| \leq k \cdot {\sf ex}(n, Z_{k+2})$, 
where $Z_k = (1,k-1, k-2, \ldots, 2, k)$. 
This gives an improvement over the previous result in two ways. First, the pattern we avoid reduces in size from $O(k^2)$ to $(k+2)$, and second the pattern $Z_k$ is simpler to analyze (``closer'' to identity).  

To our knowledge, the polynomial dependence on $k$ for ${\sf ex}(n,Z_k)$ is open, so we could not use existing theorems as a blackbox. We provide a proof that ${\sf ex}(n,Z_k) \leq n \cdot  poly(k)$, which implies Theorem~\ref{thm:main k-dec}. 
In fact, our technique allows us to derive the upper bound of ${\sf ex}(n, \pi) \leq n \cdot poly(|\pi|)$ for a broader class of permutations $\pi$ that includes $Z_k$ as a special case. 
This technique could be of independent interest (see further discussion in Section~\ref{section: k-dec}).





%In Section~\ref{sec:size3input}, we prove the bounds for preoder and postorder. Bound for $k$-decreasing sequences is proved in Section~\ref{section: k-dec}. In Section~\ref{sec:deque} we prove new bounds for deque sequence and we talk about split model in Section~\ref{section: Split}.



\vspace{0.2in} 


\noindent 
{\bf Conclusion and open problems:} 
We propose a simple idea of partitioning the execution log of Greedy into several simpler-to-analyze matrices based on the input structures and leveraging distinct patterns to upper bound each structured matrix separately.  
Based on this idea, we derived improved bounds for many notorious pattern avoidance conjectures (and completely settling the postorder conjecture).
We view these results as a showcase of the decomposition trick, which allows us to extend/strengthen the applications of forbidden submatrices in data structures. 
We believe that this technique would find further uses in BSTs and more broadly in amortized analysis of data structures. 


Our proof technique to upper bound ${\sf ex}(n,Z_k)$ might be useful in studying the classes of ``easy'' permutations whose upper bounds ${\sf ex}(n,\pi)$ grows polynomially in $|\pi|$. 
In particular, Jacob Fox~\cite{fox2013stanley} shows that there exist permutations $\pi$ such that ${\sf ex}(n, \pi) = n 2^{\Omega(k^{1/4})}$ and left open the following conjecture: 

\begin{conjecture}
If $\pi$ is a permutation that avoids $O(1)$-sized pattern, ${\sf ex}(n, \pi) = n \cdot poly(|\pi|)$. 
\end{conjecture}


Notice that our $Z_k$ avoids $(2,3,1)$ (and therefore $2$-decomposable), so it is a special case of Fox' conjecture. It is interesting to extend our proofs to handle more difficult cases.  



\vspace{0.2in} 

\noindent 
{\bf Further related works:} 
The ``parameterized'' pattern avoiding inputs, where one considers an input class whose avoided pattern has size depending on parameter $k$, have recently received attention (see e.g.,~\cite{chalermsook2015pattern,goyal2019better}). 
Research questions in this setting aim to first prove the upper bound for $\opt(X)$ as a function of $k$ and later show that Greedy matches this upper bound. 
The parameters of interest are those that generalize the classical special cases of the dynamic optimality conjecture (such as deque and pre-order traversals). 
Chalermsook et al.~\cite{chalermsook2015pattern} showed $O(n 2^{\alpha(n)^{O(|\pi|^2)}})$ upper bound for the cost of Greedy on inputs avoiding $\pi$. 
Goyal and Gupta proved $O(n \log k)$ upper bound on the cost of Greedy on $k$-decomposable sequences~\cite{goyal2019better} (if one allows ``preprocessing''). A stronger bound that subsumes the $k$-decomposable bound and the dynamic finger bound~\cite{cole2000dynamic1,cole2000dynamic2} was shown by~\cite{iacono2016weighted,bose2016power} (see discussion in~\cite{chalermsook2016landscape}.). %\footnote{Sorrachai: Probably mention Smooth Heap as a way to implement Greedy?}
Besides pattern avoidance, other BST bounds include the unified bound~\cite{buadoiu2007unified,iacono2001alternatives,derryberry2009skip} and the multi-finger bound~\cite{chalermsook2018multi,howat2013fresh,demaine2013combining}.  
The original drawback of Greedy was that, in contrast to Splay whose simplicity made it attractive for practitioners, Greedy does not admit a simple implementation in the BST model. However, due to a recent work by  Kozma and Saranurak~\cite{kozma2019smooth}, there exists a heap data structure (called smooth heap) which matches the cost of Greedy and is implementable in practice.  



%\attention{A bit about forbidden matrices. The extremal bounds for pattern of size 4 are known.}



==> tex/omitted.tex <==

\section{Proofs from Section~\ref{section: k-dec}} 






\subsection{Proof of Lemma~\ref{lem:recurrence permutation}} 

Let $M$ be a matrix that avoids $\pi$ and $|M| = \textsf{ex}(n,\pi)$. Let $n' = n/(4k^2)$. We divide the columns of $M$ into $n'$ groups of consecutive columns of size $4k^2$, and similarly we divide the rows of $M$ into $n'$ groups of  consecutive rows of size $4k^2$. Let $B_{ij}$ be the submatrix of $M$ formed by $i$-th group of columns and $j$-th group of rows respectively. We can view $M$ as a block matrix $(B_{ij})_{i,j \in [n']}$. Each block has size $(4k^2) \times (4k^2)$. We say that a row (or a column) is \textit{empty} if all entries are all zero. A matrix is \textit{empty} if all rows and columns are empty.

For each block $B_{ij}$,  we say that $B_{ij}$ is \textit{wide} if it contains at least $2k$ non-empty columns. Also, we say that $B_{ij}$ is \textit{tall} if it contains  at least $2k$ non-empty rows. Let $M'$ be the $n' \times n'$ matrix where $M'(i,j) = 1$ if and only if $B_{ij}$ is non-empty, not wide and not tall. 
Let $T$ be the $n' \times n'$ binary matrix where $T(i,j) = 1$ if and only if $B_{ij}$ is tall. Let $W$ be the $n' \times n'$ binary matrix where $W(i,j) = 1$ if and only if $B_{ij}$ is wide. Observe that each non-empty block can be tall or wide or neither, the three matrices $M'$, $T$, and $W$ covers all blocks $B_{ij}$ from $M$. 
More precisely, we have $M'(i,j) = T(i,j) = W(i,j) = 0$ if and only if $B_{ij}$ is empty. Therefore, 
\begin{align}
  |M| \leq (2k-1)^2|M'| + 16k^4|T|+16k^4|W|.  
\end{align}
The coefficient of the term $|M'|$ is $(2k-1)^2$  because the number of ones in a non-wide and non-tall block is at most $(2k-1)^2$.  The coefficient for both $T$ and $W$ is $16k^4$ because every block is $4k^2 \times 4k^2$. It remains to bound the number of 1's in $M',W$ and $T$. 

\paragraph*{The number of 1's in $M'$.}
\begin{claim}
$M'$ avoids $\pi$. Therefore, $|M'| \leq \textsf{ex}(n',\pi)$. 
\end{claim}
\begin{proof}
Suppose $M'$ contains $\pi$.  This means that there is a set of non-empty blocks $\{ B_{ij} \}$ in $M$ such that we can form the pattern $\pi$ by taking one 1's per block in the set. Therefore, $M$ contains $\pi$, a contradiction.
\end{proof}


\paragraph*{The number of 1's in $W$ and in $T$.}
\begin{claim}
$|W| \leq n'f(4k^2, \pi)$, and  $|T| \leq n'f(4k^2,\pi')$.
\end{claim}
\begin{proof}
 Since $W$ has $n'$ columns, it is enough to show that  the number of 1's in each column of $W$ is at most $f(4k^2,\pi)$. 
 We fix an arbitrary $j$-th column of $W$. Let $\ell$ be the number of 1's in the $j$-th column of $W$ (This means there are $\ell$ wide blocks in the $j$-th group of column in $M$.) 
Assume for the sake of contradiction  that $\ell > f(4k^2,\pi)$.
 
 
 
For any matrix $P$, we define the flattening of $P$ (denoted by ${\sf flat}(P)$) as a binary row-vector $v$, where $v(k) = 1$ if and only if $k$-th column of $P$ is non-empty. 
Let $Q_j$ be the binary matrix obtained by flattening of all the blocks in the $j$-th column-group. More formally, matrix $Q_j$ has $(4k^2)$ columns and $n'$ rows where each row $i \in [n']$ is a flattening of $B_{ij}$. 

\begin{observation}
If $Q_j$ contains permutation $\pi$, then $M$ contains $\pi$. 
\end{observation}

Observe that the number of 1's in each row of $Q_j$ is at least $2k$ because $B_{ij}$ is wide.  Since $\ell > f(4k^2,\pi)$, and each row of $Q_j$ has at least $2k$ many 1's,  Definition \ref{def:long vector pattern} implies that $Q_j$ contains $\pi$, which implies that $M$ contains $\pi$, a contradiction.  
%By definition of $Q_i$, $\text{vec}(B_{i,r_1}), \ldots, \text{vec}(B_{i,r_k})$ form a submatrix of $Q_i$ that contains $\pi$. By definition of $\text{vec}(B_{i,j})$, the blocks $B_{i,r_1}, B_{i,r_2}, \ldots, B_{i,r_k}$ form a submatrix of $M$ that contains $\pi$.  Therefore, $M$ contains $\pi$, a contradiction. Therefore, the number of 1's in the $i$-th column of $W$ is $\ell \leq f(4k^2,\pi)$. The argument for $| T| \leq n'f(4k^2,\pi')$ is similar, but we need the rotated pattern $\pi'$ instead of $\pi$. 
\end{proof}


\subsection{Proof of Lemma~\ref{cor:ex and f}}

Let $T(n) = \textsf{ex}(n,\pi)$, $q = 4k^2$, and $g(q) = f_{2}(q,\pi)+f_{2}(q,\pi')$. By \Cref{lem:recurrence permutation}, we have 
\begin{align*}
    T(n) &\leq (2k-1)^2T(n/q) + nq(g(q)) \\
    & \leq nq(g(q)) + \frac{(2k-1)^2}{q}nq(g(q)) + (\frac{(2k-1)^2}{q})^2 nq(g(q)) + \ldots  \\ 
    & \leq nq(g(q)) (\sum_{i\geq 0}(\frac{(2k-1)^2}{q})^i) \\ 
    &\leq nq(g(q))k.
\end{align*}
The last inequality follows since $(2k-1)^2/q = (2k-1)^2/(4k^2) < 1$. 

